Hide and Seek: How Does Watermarking Impact Face Recognition?

The recent progress in generative models has revolutionized the synthesis of highly realistic images, including face images. This technological development has undoubtedly helped face recognition, such as training data augmentation for higher recognition accuracy and data privacy. However, it has also introduced novel challenges concerning the responsible use and proper attribution of computer generated images. We investigate the impact of digital watermarking, a technique for embedding ownership signatures into images, on the effectiveness of face recognition models. We propose a comprehensive pipeline that integrates face image generation, watermarking, and face recognition to systematically examine this question. The proposed watermarking scheme, based on an encoder-decoder architecture, successfully embeds and recovers signatures from both real and synthetic face images while preserving their visual fidelity. Through extensive experiments, we unveil that while watermarking enables robust image attribution, it results in a slight decline in face recognition accuracy, particularly evident for face images with challenging poses and expressions. Additionally, we find that directly training face recognition models on watermarked images offers only a limited alleviation of this performance decline. Our findings underscore the intricate trade off between watermarking and face recognition accuracy. This work represents a pivotal step towards the responsible utilization of generative models in face recognition and serves to initiate discussions regarding the broader implications of watermarking in biometrics.

==> sec/0_outline.tex <==

\begin{center}
    \textbf{Outline of the paper}
\end{center}


\textbf{Deadline: 19th March}

\begin{enumerate}
\item{Introduction}
\begin{enumerate}
    \item Real imgaes / fake images on the internet and their impact on the face recognition models.
    \item Background on face recognition technology
    \item Generated images to boost the performance of face recognition technology
    \item Watermarking as a potential solution for image authentication and ownership protection
    \item Research question:
    \begin{center}
    \textbf{\textit{Will the watermarked facial images affect the performance of face recognition models?}}
    \end{center}    
    \item One-sentence summary:
    \begin{center}
    \YY{\textbf{\textit{The watermarked facial images have weak effects on the performance of face recognition models? Or they have strong effects?}}}
    \end{center} 

    1. watermarked image visibility?
    
    2. biometric matching results?
    
    3. robustness of transformation?
    
    4. watermarked synthetic data used for training face recognition?

    5. Reverse engineer of the watermark? Denoising process over the watermarked images? What factors needed by the attackers?
    
    
\end{enumerate}

\item{Related Work}
\begin{enumerate}
    \item Overview of existing face recognition techniques and their performance. Studies on the impact of image distortions on face recognition. Studies on the impact of generated images on face recognition.
    \item Applications of watermarking in image authentication and copyright protection. Watermarked generated images to protect the copyright. Gaps in the literature and motivation for the current study. \textbf{no one peers into the watermarked images trained face recognition model.}
\end{enumerate}

\item{Method}
\begin{enumerate}
    \item Dataset description and preprocessing
    \item Watermarking techniques employed (With method details)
    \begin{enumerate}
        \item Invisible watermarking: DCT/DWT (Frequency-based) and \textbf{HIDDEN} (CNN-based). We can focus on \textbf{one watermarking technology}.
        \item How to adapt these images for face recognition model training. 
    \end{enumerate}
    \item Face recognition models used for evaluation and the generation methods (like DCFace) for Face recognition models.
    \item Performance metrics and evaluation protocol

\end{enumerate}

\item{Experiment}
\begin{enumerate}
    \item Experimental setup and parameter settings
    \item Different watermarking visualization
    \item \textbf{effectiveness of watermarking. Face matching? Augmentation? }
    \item Impact of visible/invisible watermarks on face recognition performance
    \item \textbf{influence results corresponding to face recognition.}
\end{enumerate}




\item{Conclusion}
\end{enumerate}

==> sec/2_introduction.tex <==
\section{Introduction}

We ask:

\begin{center}
    \textit{\textbf{(Q)} 
Can face recognition models trained on watermarked synthetic data maintain their effectiveness?
}
\end{center}


\paragraph{Contributions.} We summarize our main contributions as below.

$\bullet$

$\bullet$

$\bullet$


==> sec/4_problem_statement.tex <==
\section{Preliminaries and Problem Statement}

% \SL{[A problem statement section is missing. E.g., Preliminaries and Problem Statement]}

In this section, we introduce the motivation and problem setup for watermarking generated face images in the context of training face recognition models. We first provide an overview of digital watermarking. Then, we discuss the preliminaries of diffusion models for face generation. Finally, we introduce the face recognition task and conclude the key problem addressed in this work.

\paragraph{Digital Watermarking.}
Digital watermarking is a technique used to embed hidden information, called a watermark, into digital content such as images, audio, or video. The primary purpose of watermarking is to protect the intellectual property rights of the content owner and ensure the authenticity and integrity of the digital asset. Watermarks can be designed to be invisible to the human eye while being detectable by specialized algorithms. In the context of generated face images, watermarking can be used to trace the origin of the images and prevent unauthorized use or distribution.

The watermarking problem can be formulated as follows: given an input image $\mathbf{I} \in \mathbb{R}^{H \times W \times C}$ and a binary watermark message $\mathbf{m} \in \{0, 1\}^L$ where $L$ is the bit string length, the goal is to generate a watermarked image $\mathbf{I}_w$ that visually resembles the original image while embedding the watermark message. The watermarked image should be resilient to common image transformations, such as compression, resizing, and cropping, while allowing reliable extraction of the watermark message.

To achieve this, we can employ deep neural networks as proposed in the HiDDeN framework \cite{zhu2018hidden}. The watermarking system consists of an encoder network $f_{\theta}$ and a decoder network $g_{\phi}$. The encoder takes the input image $\mathbf{I}$ and the watermark message $\mathbf{m}$ as inputs and generates the watermarked image $\mathbf{I}_w = f_{\theta}(\mathbf{I}, \mathbf{m})$. The decoder takes the watermarked image $\mathbf{I}_w$ as input and extracts the embedded watermark message $\hat{\mathbf{m}} = g_{\phi}(\mathbf{I}_w)$.

The encoder and decoder networks are trained jointly using a combination of image reconstruction loss and message decoding loss. The image reconstruction loss ensures that the watermarked image is visually similar to the original image, while the message decoding loss minimizes the difference between the embedded and extracted watermark messages. The training objective can be formulated as:

\begin{equation}
\min_{\theta, \phi} \mathcal{L}_{\mathrm{img}}(f_{\theta}(\mathbf{I}, \mathbf{m}), \mathbf{I}) + \lambda \mathcal{L}_{\mathrm{mes}}(g_{\phi}(f_{\theta}(\mathbf{I}, \mathbf{m})), \mathbf{m}),
\end{equation}

where $\mathcal{L}_{\mathrm{img}}$ is the image reconstruction loss (e.g., mean squared error, MSE), $\mathcal{L}_{\mathrm{mes}}$ is the message decoding loss (e.g., binary cross-entropy loss per bit, BCE), and $\lambda$ is a hyperparameter balancing the two loss terms.

\paragraph{Face generation through diffusion models.}
Diffusion models have emerged as a powerful approach for generating high-quality face images. These models learn to generate realistic faces by gradually denoising a Gaussian noise signal through a series of denoising steps. The denoising process is guided by a learned noise schedule, which determines the amount of noise to be removed at each step. Diffusion models have shown impressive results in generating diverse and visually appealing face images, making them a promising tool for data augmentation and synthetic dataset creation.

In this work, we employ DCFace \cite{kim2023dcface}, a state-of-the-art diffusion-based face generation model. DCFace builds upon the success of diffusion models and introduces several key innovations to enhance the quality and controllability of generated face images conditioned on individual identities and face variations.  DCFace consistently produces face images of the same identity under different styles with precise control, providing face recognition models with augmented training data of higher variations. 

\paragraph{Face recognition.} 
Face recognition is a biometric technology that aims to identify or verify individuals based on their facial features. It has numerous applications, including security systems, surveillance, and user authentication. Deep learning-based face recognition models have achieved remarkable performance by learning discriminative features from large-scale face datasets \cite{zhu2021webface260m, guo2016ms}. However, collecting and annotating real face images can be time-consuming and challenging due to privacy concerns and data acquisition costs. Generated face images offer a potential solution to augment training data and improve the robustness of face recognition models. 

In this work, we focus on the face recognition model setup similar to AdaFace \cite{kim2022adaface}. Given an input face image $\mathbf{I} \in \mathbb{R}^{H \times W \times C}$,  a face recognition model $f_{\theta}$ maps the image to a compact feature representation $\mathbf{x} \in \mathbb{R}^{d}$:

\begin{equation}
\mathbf{x} = f_{\theta}(\mathbf{I}),
\end{equation}

where $\theta$ represents the learnable parameters of the model. The feature representation $\mathbf{x}$ is typically obtained from the penultimate layer of a deep convolutional neural network (CNN) architecture, such as ResNet \cite{he2016deep} or MobileFaceNet \cite{chen2018mobilefacenets}.

To train the face recognition model, a large-scale dataset with identity labels is used. Let $\mathcal{D} = \{(\mathbf{I}_i, y_i)\}_{i=1}^{N}$ be the training dataset, where $\mathbf{I}_i$ is the $i$-th face image and $y_i \in \{1, 2, \dots, K\}$ is the corresponding identity label, with $K$ being the total number of identities in the dataset. The model is trained to minimize a classification loss, such as the softmax loss \cite{deng2019arcface} or the margin-based loss \cite{liu2017sphereface, wang2018cosface, deng2019arcface}, which encourages the features of faces from the same identity to be close together in the embedding space while pushing apart the features of faces from different identities.

During inference, the face recognition model extracts the feature representation $\mathbf{x}_p$ for a probe face image $\mathbf{I}_p$. The similarity between the probe face and a reference face $\mathbf{I}_r$ with feature representation $\mathbf{x}_r$ is computed using a similarity metric, such as the cosine similarity:

\begin{equation}
s(\mathbf{x}_p, \mathbf{x}_r) = \frac{\mathbf{x}_p^T \mathbf{x}_r}{|\mathbf{x}_p| |\mathbf{x}_r|},
\end{equation}

where $|\cdot|$ denotes the Euclidean norm. The probe face is considered to match the reference face if their similarity score exceeds a predefined threshold $\tau$:

\begin{equation}
\text{match}(\mathbf{x}_p, \mathbf{x}_r) = 
\begin{cases}
1, & \text{if } s(\mathbf{x}_p, \mathbf{x}_r) \geq \tau, \\
0, & \text{otherwise}.
\end{cases}
\end{equation}

The performance of face recognition models is typically evaluated using metrics such as verification accuracy, true acceptance rate (TAR) at a fixed false acceptance rate (FAR), and equal error rate (EER) on benchmark datasets like LFW \cite{huang2008labeled}, CFP-FP \cite{sengupta2016frontal}, and AgeDB \cite{moschoglou2017agedb}.

By augmenting the training data with generated face images that exhibit diverse variations in pose, expression, illumination, and other factors, the robustness and generalization ability of face recognition models can be improved. In this work, we leverage the DCFace \cite{kim2023dcface} model to generate high-quality synthetic face images for training face recognition models, aiming to enhance their performance and resilience to various real-world scenarios.

\paragraph{Problem statement.}
The key problem studied in this work is the watermarking of generated face images for training face recognition models. We aim to develop a watermarking scheme that embeds a robust and imperceptible watermark into the generated face images while preserving their visual quality and utility for face recognition tasks. The watermark should be resilient to common image transformations and detectable even after the images have been used to train a face recognition model. By watermarking the generated face images, we seek to establish ownership, prevent misuse, and enable traceability of the synthetic data. Additionally, we investigate the impact of watermarking on the performance of face recognition models trained and evaluated using the watermarked images.

==> sec/5_method.tex <==
\section{Methods}
In this section, we present the details of our proposed approach that combines watermarking techniques with face recognition model training. Our methodology consists of three main components: (1) watermarking network to encode binary bits into the images, (2) synthetic face image generation via the diffusion model, and (3) training a face recognition model using the watermarked synthetic images. We assess the feasibility of the watermarking method through its invisibility and bit accuracy, which measures the percentage of correctly decoded bits. To evaluate the impact of watermarking on the synthetic data trained face recognition model, we demonstrate the corresponding recognition model training, and the evaluation metrics used to measure the performance. 

\begin{figure*}[!t]
\includegraphics[width=\textwidth,height=!]{fig/pipeline.pdf}
\vspace{-5mm}
\caption{\footnotesize{
{Overview of watermarking encoder/extractor training (left) and the pipeline of generated face watermarking for face recognition (right).
\SL{[Needs improvement! We can talk tomorrow.]}
}
}}
 \vspace*{-3mm}
\label{fig: pipeline}
\end{figure*}

\subsection{Watermarking encoder and extractor.}
In this study, we employ the Hidden Deniable Distortion Network (HiDDeN) \cite{zhu2018hidden} method for watermarking face images. HiDDeN is a deep learning-based approach that enables the embedding of binary-string watermarks into images while maintaining a high level of visual fidelity and robustness against various attacks. 

\paragraph{Network architecture and watermarking string design.}
To embed the bit string into images by the watermarking encoder $f_{\theta}$, we first project the bit string and the input image into the same dimension. After concatenating the projected bit string and the input image, we feed them into a series of convolutional layers followed by residual blocks. The encoder eventually outputs the watermarked image $\mathbf{I}_w$, which has the same dimensions as the input image. 

The watermarking extractor $g_{\phi}$ takes the watermarked image as input and passes it through a series of blocks and a linear layer with output equal to the bit string length to extract the embedded watermark message. The extractor outputs a predicted bit string $\hat{\mathbf{m}}$, which is then compared with the original bit string $\mathbf{m}$ to compute the watermark extraction loss. 

During the watermarking encoder/extractor training, for each training image, an $L$-bit string is randomly generated and embedded into the image. This random bit string generation helps the encoder and extractor learn to handle diverse watermark patterns and prevents overfitting to specific bit sequences (See the illustration in Fig.\,\ref{fig: pipeline}). Then for the actual use to watermark face images, we assign a fixed $L$-bit string, as a unique identifier for the generated images by a specific model authority.

\paragraph{Robustness of watermark through data augmentation.} To enhance the robustness of the watermarking system, the HiDDeN framework incorporates data augmentations during training. The input images and watermarked images are subjected to various image transformations, such as random cropping, resizing, and compression, to simulate real-world scenarios. By training the encoder and decoder networks with augmented data, the watermarking system learns to embed and extract watermarks that are resilient to these transformations. This makes it a suitable approach for watermarking generated face images, ensuring their traceability and preventing unauthorized use or distribution.

\subsection{Synthetic face generation.}
\YY{merged into the preliminaries.}
As for synthetic face generation, we follow the Dual Condition Diffusion Model (DCFace) \cite{kim2023dcface} to generate multiple styles for each individual identity. The resulted synthetic dataset can help face recognition model training and is proven to be the state of the art to minimize the recognition performance gap compared to the real dataset. 

\paragraph{Face generation objectives in diffusion models: diversity and consistency.}

\paragraph{Two-stage conditional face generation.}

\subsection{Face recognition model and evaluation metrics.}
We then train the face recognition model over the watermarked synthetic face images. 

\paragraph{Face matching via the embedding similarity.}

\paragraph{Face recognition model architecture.}









